Cover Semantics for Intuitionistic Modalities

Intuitionistic modal logic (IML) has inspired several developments in programming languages including modal type systems for staging, computational effects and language-based security. IMLs are typically studied using Kripke-style relational semantics, which simplifies proofs of meta-theoretic properties, such as completeness and consistency, by making it easy to construct models. Kripke-style relational semantics, however, relies upon classical reasoning principles, which makes it unappealing from a computational perspective and unsuitable for formalization in a constructive type theory. Goldblatt provides an alternative semantics for IMLs by extending Beth-Kripke-Joyal-style "cover" semantics for intuitionistic propositional logic with relations to support modalities. Goldblatt's "relational cover" semantics overcomes classical reasoning but introduces a new limitation: it relies upon a "modal localization" condition that restricts the class of models and complicates model construction. Goldblatt bypasses this restriction by using intricate order-theoretic completion arguments to prove completeness. In this article, we present a conservative extension of relational cover semantics that alleviates this restriction and is amenable to simpler and standard model construction techniques. We formalize our semantics in Agda and prove completeness constructively in the style of Normalization by Evaluation for a variety of IMLs featuring independent box and diamond modalities.

==> lib/macros.tex <==
\makeatletter
\DeclareRobustCommand{\mycircle}{\mathord{\mathpalette\is@circle\relax}}
\newcommand\is@circle[2]{%
  \begingroup
  \sbox\z@{\raisebox{\depth}{$\m@th#1\bigcirc$}}%
  \sbox\tw@{$#1\square$}%
  \resizebox{!}{\ht\tw@}{\usebox{\z@}}%
  \endgroup
}
\makeatother



%\DeclareSymbolFont{system}{T1}{cmr}{m}{sc}
\makeatletter
\def\system@font{\rmfamily}
\def\systemfont{\system@font}
\NewDocumentCommand{\DeclareSystem}{mmm}{%
  \expandafter\DeclareRobustCommand\expandafter{\csname#1\endcsname}{{\system@font\glsfmttext{#1}}\xspace}
  \expandafter\DeclareRobustCommand\expandafter{\csname#1s\endcsname}{{\system@font\glsentryplural{#1}}\xspace}
  \newglossaryentry{#1}{%
    name={#2},
    description={#3}
  }
}
\makeatother

\makeatletter
\NewDocumentCommand\dependson{mom}{%
  \@ifpackageloaded{#1}{%
    #3
  }{%
    \IfValueTF{#2}{
      \PackageWarningNoLine{macros}{Load package `#1' for #2}
    }{%
      \PackageWarningNoLine{macros}{Package `#1' needed for some macros but missing}
    }
  }
}
\NewDocumentCommand\dependsoncommand{mom}{%
  \ifcsname #1\endcsname
    #3
  \else
    \IfValueTF{#2}{
      \PackageWarningNoLine{macros}{Define command `#1' for #2}
    }{%
      \PackageWarningNoLine{macros}{Command `#1' needed for some macros but missing}
    }
  \fi
}
\makeatother

\NewDocumentCommand{\thyeq}{}{\sim} % axiomatic equality (of an equational theory, in a quotient, any congruence relation)

% type operators
\NewDocumentCommand{\MonPr}{g}{\heartsuit\IfValueT{#1}{#1}}
\NewDocumentCommand{\BoxPr}{g}{\square\IfValueT{#1}{#1}}
\NewDocumentCommand{\DiaPr}{g}{\lozenge\IfValueT{#1}{#1}}
\NewDocumentCommand{\LaxPr}{g}{\lozenge\IfValueT{#1}{#1}}
\DeclareTypeInfix{\ImpPr}{\Rightarrow}
\DeclareTypeInfix{\AndPr}{\land}
\DeclareTypeInfix{\OrPr}{\lor}
\NewDocumentCommand{\BlackDiaPr}{g}{\blacklozenge\IfValueT{#1}{#1}}

% term operators

\DeclareTermConstant{\zeroVar}{zero}

\DeclareTermOperator{\succVar}{succ}
\DeclareTermOperator{\varTm}{var}
\DeclareTermOperator{\lamTm}{\lambda}
\DeclareTermOperator{\appTm}{app}
\DeclareTermOperator{\unitTm}{unit}
\DeclareTermOperator{\pairTm}{pair}
\DeclareTermOperator{\fstTm}{fst}
\DeclareTermOperator{\sndTm}{snd}
\DeclareTermOperator{\returnLLTm}{return_{\text{\LL}}}
\DeclareTermOperator{\letLLTm}{let_{\text{\LL}}}
\DeclareTermOperator{\letSLTm}{letmap_{\text{\SL}}}
\DeclareTermOperator{\letRLTm}{letmap_{\text{\RL}}}
\DeclareTermOperator{\letMapJLTm}{letmap_{\text{\JL}}}
\DeclareTermOperator{\letJoinJLTm}{let_{\text{\JL}}}
\DeclareTermOperator{\returnRLTm}{return_{\text{\RL}}}
\DeclareTermOperator{\succVar}{succ}
\DeclareTermOperator{\upTm}{up}


\DeclareTermOperator{\fmapHTm}{fmap}
\DeclareTermOperator{\returnHTm}{return}
\DeclareTermOperator{\joinHTm}{join}

% keywords

\DeclareTermOperator{\inKw}{in}


% context operators
\DeclareTermConstant{\EmptyCtx}{{\cdot}}
\NewDocumentCommand{\ExtCtx}{mm}{#1, #2}
\NewDocumentCommand{\ProdCtx}{mm}{#1, #2}
\NewDocumentCommand{\DualCtx}{mm}{#1 \,;\, #2}
\DeclareTypeConstant{\LockCtx}{\textnormal{\faLock}}
\NewDocumentCommand{\LockedCtx}{m}{\ExtCtx{\Gamma}{\LockCtx}}

% for contexts
\NewDocumentCommand{\Wk}{mm}{#1 \leq #2}

% for extensions
\DeclareTermOperator{\nilExt}{nil}
\DeclareTermOperator{\varExt}{cons}
\DeclareTermOperator{\varExtOnce}{single}

% for domains of a typed lambda calculus model
\DeclareMathConstant{\Ctx}{Ctx}
\DeclareMathConstant{\Ty}{Ty} % nondependent types
\NewDocumentCommand{\Tm}{mm}{#1 \vdash #2} % don't \DeclareMathInfix in case the prefix notation Tm(Γ,A) will be preferred
\NewDocumentCommand{\Ne}{mm}{#1 \vdashNe #2} % ditto
\NewDocumentCommand{\Nf}{mm}{#1 \vdashNf #2} % ditto
% \NewDocumentCommand{\Subst}{mm}{#1 \vdashSub #2} % ditto
\DeclareMathConstant{\Type}{Type}
\DeclareMathConstant{\Prop}{Prop}
\DeclareMathConstant{\Atom}{Atom}

% systems
\DeclareSystem{CPL}{CPL}{}
\DeclareSystem{IPL}{IPL}{}
\DeclareSystem{IPLNeg}{$\text{IPL}_{\top,\times,\Rightarrow}$}{}
\DeclareSystem{CM}{CM}{} % constructive monotone modal logic
\DeclareSystem{CK}{CK}{} % constructive K
\DeclareSystem{HKDia}{$\text{HK}_{\DiaPr{}}$}{} %
\DeclareSystem{WK}{WK}{} % Wijesekera's
\DeclareSystem{IK}{IK}{} % Wijesekera's 

\DeclareSystem{SL}{SL}{}
\DeclareSystem{RL}{SRL}{}
\DeclareSystem{JL}{SJL}{}
\DeclareSystem{LL}{PLL}{}

\DeclareSystem{CKBox}{CK$_{\BoxPr{}}$}{} % constructive K with boxes
\DeclareSystem{CSFour}{CS4}{}
\DeclareSystem{CKDia}{CK$_{\DiaPr{}}$}{} % constructive K with diamonds
\DeclareSystem{CSFourBox}{CS4$_{\BoxPr{}}$}{} % constructive K
\DeclareSystem{DCKBox}{D\CKBox}{} % Dual-context constructive K
\DeclareSystem{FCKBox}{F\CKBox}{} % Fitsh-style constructive K
\DeclareSystem{DCSFourBox}{D\CSFourBox}{}

\DeclareSystem{STLC}{STLC}{}
\DeclareSystem{SLC}{\protect\textnormal{\textlambda}\textsubscript{\SL}}{}
\DeclareSystem{RLC}{\protect\textnormal{\textlambda}\textsubscript{\RL}}{}
\DeclareSystem{JLC}{\protect\textnormal{\textlambda}\textsubscript{\JL}}{}
\DeclareSystem{LLC}{\protect\textnormal{\textlambda}\textsubscript{\LL}}{}

%\NewDocumentCommand{\Cp}{}{\mathcal{C}_+}
%\NewDocumentCommand{\Cm}{}{\mathcal{C}_{\LaxTy{}}}
\NewDocumentCommand{\Ri}{mm}{#1 \sqsubseteq #2}
\NewDocumentCommand{\RiOp}{mm}{#1 \sqsupseteq #2}
\NewDocumentCommand{\Rin}{mm}{#1 \preceq #2}
\NewDocumentCommand{\RinOp}{mm}{#1 \succeq #2}

\DeclareMathOperator{\reflRi}{refl_{i}}
\DeclareMathOperator{\transRi}{trans_{i}}
\NewDocumentCommand{\Rm}{}{\mathrel{R}}
\NewDocumentCommand{\RmBox}{}{\mathrel{R}_{\BoxPr}}
\NewDocumentCommand{\RmDia}{}{\mathrel{R}_{\DiaPr}}
\NewDocumentCommand{\RmOp}{}{\mathrel{R}^{-1}}
\NewDocumentCommand{\RCM}{}{\Rm_\text{\CM}}

\DeclareMathOperator{\reflRm}{refl_{m}}
\DeclareMathOperator{\transRm}{trans_{m}}
\DeclareMathOperator{\incl}{incl}

\NewDocumentCommand{\Covp}{mm}{#1 \vartriangleleft #2}
\NewDocumentCommand{\CovpOp}{mm}{#1 \vartriangleright #2}
\NewDocumentCommand{\Covm}{mm}{#1 \blacktriangleleft #2}
\NewDocumentCommand{\CovmOp}{mm}{#1 \blacktriangleright #2}

% Instances
\NewDocumentCommand{\CovpIPL}{mm}{#1\vartriangleleft_{\text{\IPL}}#2}
\NewDocumentCommand{\CovpIPLOp}{mm}{#1\vartriangleright_{\text{\IPL}}#2}
\NewDocumentCommand{\CovmCM}{mm}{#1\blacktriangleleft_{\text{\CM}}#2}
\NewDocumentCommand{\CovmCMOp}{mm}{#1\blacktriangleright_{\text{\CM}}#2}
\NewDocumentCommand{\CovmSL}{mm}{#1\blacktriangleleft_{\text{\SL}}#2}
\NewDocumentCommand{\CovmSLOp}{mm}{#1\blacktriangleright_{\text{\SL}}#2}
\NewDocumentCommand{\CovmLL}{mm}{#1\blacktriangleleft_{\text{\LL}}#2}
\NewDocumentCommand{\CovmLLOp}{mm}{#1\blacktriangleright_{\text{\LL}}#2}
%
\NewDocumentCommand{\CovpDCKBox}{mm}{#1\vartriangleleft_{\text{\DCKBox}}#2}
\NewDocumentCommand{\CovmDCKBox}{mm}{#1\blacktriangleleft_{\text{\DCKBox}}#2}
%
\NewDocumentCommand{\CovpDCSFourBox}{mm}{#1\vartriangleleft_{\text{\DCSFourBox}}#2}
\NewDocumentCommand{\CovmDCSFourBox}{mm}{#1\blacktriangleleft_{\text{\DCSFourBox}}#2}
%
\NewDocumentCommand{\CovmDCKBoxOp}{mm}{#1\blacktriangleright_{\text{\DCKBox}}#2}
\NewDocumentCommand{\CovmFCKBox}{mm}{#1\blacktriangleleft_{\text{\FCKBox}}#2}
\NewDocumentCommand{\CovmFCKBoxOp}{mm}{#1\blacktriangleright_{\text{\FCKBox}}#2}

%

\NewDocumentCommand{\Pow}{}{\mathcal{P}}
\NewDocumentCommand{\LUp}{}{\mathcal{LU}}
\NewDocumentCommand{\Up}{}{\mathcal{U}}

\NewDocumentCommand{\uOp}{}{\uparrow}
\NewDocumentCommand{\jOp}{}{\langle\Covp{}{}\rangle}
\NewDocumentCommand{\mOp}{}{\langle\Covm{}{}\rangle}
\NewDocumentCommand{\rOp}{}{\langle\Rm\rangle}

\DeclareMathOperator{\AntTh}{Ant}
\DeclareMathOperator{\NfTh}{Nf}
\DeclareMathOperator{\NeTh}{Ne}
\DeclareMathOperator{\N}{N}

% axioms
\def\KA    {\TirName{K}\xspace}
\def\SA    {\TirName{S}\xspace}
\def\RA    {\TirName{R}\xspace}
\def\JA    {\TirName{J}\xspace}
\def\TA    {\TirName{T}\xspace}
\def\FourA {\TirName{4}\xspace}

% for derivations
\NewDocumentCommand{\vdashVar}{}{\vdash_{\textsc{var}}}
\NewDocumentCommand{\vdashNf}{}{\vdash_{\textsc{nf}}}
\NewDocumentCommand{\vdashNe}{}{\vdash_{\textsc{ne}}}
\NewDocumentCommand{\vdashSub}{}{\vdash_{\textsc{s}}}

% frames
\NewDocumentCommand{\pr}{}{{\fontfamily{qtm}\selectfont pr}}

\DeclareTypeConstant{\TopPr}{\top}
\DeclareTypeConstant{\BotPr}{\bot}
\DeclareTypeOperator{\ArrTy}{Array}
\DeclareTypeOperator{\WriterTy}{Writer}
\DeclareTypeOperator{\StateTy}{State}
\DeclareTypeOperator{\MaybeTy}{Maybe}
\DeclareTypeOperator{\ExceptTy}{Except}

\dependson{mathtools}[\string\eval]{%
  \let\evallbracket\llbracket
  \let\evalrbracket\rrbracket
  \DeclarePairedDelimiter\eval\evallbracket\evalrbracket
}

\DeclarePairedDelimiter{\truth}{|}{|}

\let\quote=\relax
\DeclareMathOperator{\quote}{quote}
\DeclareMathOperator{\reify}{reify}
\DeclareMathOperator{\reflect}{reflect}
\DeclareMathOperator{\reifyR}{reifyAcc}
\DeclareMathOperator{\norm}{norm}
\DeclareMathOperator{\lookup}{lookup}
\DeclareMathOperator{\idEnv}{idEnv}


% for weakenings
\DeclareMathConstant{\baseWk}{base}
\DeclareMathOperator{\dropWk}{drop}
\DeclareMathOperator{\keepVarWk}{keep}
\DeclareMathOperator{\keepLockWk}{keep_{\lockCtx}}
\NewDocumentCommand{\subst}{mm}{#1 [#2]}
\DeclareMathOperator{\wk}{wk}
\DeclareMathConstant{\idWk}{refl_{\leq}}
\DeclareMathOperator{\transWk}{trans_{\leq}}
\DeclareMathConstant{\dropIdWk}{new}

% Categorical stuff


\NewDocumentCommand{\CircFun}{g}{\mycircle\IfValueT{#1}{#1}}
\NewDocumentCommand{\CircMap}{g}{\mycircle\IfValueT{#1}{#1}}

\NewDocumentCommand{\DiaFun}{g}{\lozenge\IfValueT{#1}{#1}}
\NewDocumentCommand{\DiaMap}{g}{\lozenge\IfValueT{#1}{#1}}
\DeclareTypeInfix{\FunFun}{\Rightarrow}
\DeclareTypeInfix{\ProdFun}{\times}

\DeclareTypeInfix{\Prod}{\times}

\NewDocumentCommand{\FFun}{g}{F\IfValueT{#1}{#1}}
\NewDocumentCommand{\FMap}{g}{F\IfValueT{#1}{#1}}

\NewDocumentCommand{\Fork}{gg}{\langle{#1},{#2}\rangle}

% for metavariables ranging over presheaves we use \mathcal
\NewDocumentCommand{\mcA}{}{\mathcal{A}}
\NewDocumentCommand{\mcB}{}{\mathcal{B}}

% for metavariables ranging over (categorical) models we use \mathcal
\NewDocumentCommand{\mcC}{}{\mathcal{C}}
\NewDocumentCommand{\mcM}{}{\mathcal{M}}
\NewDocumentCommand{\mcN}{}{\mathcal{N}}

% logical relations
\DeclareMathOperator{\LR}{L}

